CTI4AI: Threat Intelligence Generation and Sharing after Red Teaming AI Models

As the practicality of Artificial Intelligence (AI) and Machine Learning (ML) based techniques grow, there is an ever increasing threat of adversarial attacks. There is a need to red team this ecosystem to identify system vulnerabilities, potential threats, characterize properties that will enhance system robustness, and encourage the creation of effective defenses. A secondary need is to share this AI security threat intelligence between different stakeholders like, model developers, users, and AI/ML security professionals. In this paper, we create and describe a prototype system CTI4AI, to overcome the need to methodically identify and share AI/ML specific vulnerabilities and threat intelligence.

==> table.tex <==

% INCLUDE FIGURES FOR 0.2 and 0.017
\begin{table}[h]
    \centering
    \begin{tabular}{llll}
        \includegraphics[width=.2\linewidth]{Pictures/unperturbed_image_0.png}  \includegraphics[width=.2\linewidth]{Pictures/unperturbed_image_1.png} 
        \includegraphics[width=.2\linewidth]{Pictures/unperturbed_image_2.png} 
        \includegraphics[width=.2\linewidth]{Pictures/unperturbed_image_3.png}\\

        \includegraphics[width=.2\linewidth]{Pictures/perturbed_image_0.png}  \includegraphics[width=.2\linewidth]{Pictures/perturbed_image_1.png} 
        \includegraphics[width=.2\linewidth]{Pictures/perturbed_image_2.png} 
        \includegraphics[width=.2\linewidth]{Pictures/perturbed_image_3.png}\\
    \end{tabular}
    \caption{Example inputs for the CIFAR-10 model. Top row is unperturbed and bottom row is perturbed using ART with 0.017 epsilon parameter setting.}
    \label{fig2}
    \vspace{-5mm}
\end{table}

